Provable Weak-to-Strong Generalization via Benign Overfitting

The classic teacher-student model in machine learning posits that a strong teacher supervises a weak student to improve the student's capabilities. We instead consider the inverted situation, where a weak teacher supervises a strong student with imperfect pseudolabels. This paradigm was recently brought forth by Burns et al.'23 and termed \emph{weak-to-strong generalization}. We theoretically investigate weak-to-strong generalization for binary and multilabel classification in a stylized overparameterized spiked covariance model with Gaussian covariates where the weak teacher's pseudolabels are asymptotically like random guessing. Under these assumptions, we provably identify two asymptotic phases of the strong student's generalization after weak supervision: (1) successful generalization and (2) random guessing. Our techniques should eventually extend to weak-to-strong multiclass classification. Towards doing so, we prove a tight lower tail inequality for the maximum of correlated Gaussians, which may be of independent interest. Understanding the multilabel setting reinforces the value of using logits for weak supervision when they are available.

==> multiclass-proofs.tex <==

%!TEX root = ./main.tex

% \section{Binary classification}
% We now study which regimes we can satisfy the desiderata for binary classification, and more generally the case where we have $k = O(1)$ classes.
% \begin{lemma}
%     Assume that the strong learner is drawn from the $(p, q, r, 0)$-bilevel ensemble scaled to $n$ and that the weak learner is drawn from $(p_{\weak}, q_{\weak}, r_{\weak}, 0)$-bilevel ensemble scaled to $n$. 
%     Assume that the weak learner outputs labels which have independent label noise with some constant correlation $\rho > 0$.

%     Then, the desiderata are satisfied if the following conditions hold:
%         \begin{align*}
%             \max\qty{\frac{p+1}{2}, u} &< q + r < \frac{p + u}{2}
%         \end{align*}
%     In particular, this is non-vacuous if $p > u$, which is reasonable since we assume that the unlabeled finetuning set is still small relative to the strong learner.
% \end{lemma}
% \begin{proof}
%     With $n$ unlabeled datapoints, and parameters $(p, q, r, t)$ \emph{scaled to} $n$, the conditions for not being able to see the spike are 
%     \[
%         q+r > 1.  
%     \]
%     In this case, we actually have $m + n \sim n^u$ unlabeled datapoints. 
%     Let us set some notation to distinguish between the scaling of the strong learner with respect to $n$ and with respect to $m$. 
%     We will write $(p_n, q_n, r_n, t_n) \leftarrow (p, q, r, t)$, whereas $(p_m, q_m, r_m, t_m) \leftarrow (\tfrac{p}{u}, \tfrac{q}{u}, \tfrac{r}{u}, \tfrac{t}{u})$.

%     Hence relative to $m$, the strong learner is drawn from the $(p_m, q_m, r_m, u_m)$ ensemble, whereas the weak learner is drawn from $(p_{\weak}/u, q_{\weak}/u, r_{\weak}/u, t/u)$. 
%     We thus want the $q_{\weak} + r_{\weak} > u$ to ensure that we can't see the spike in the weak learner. 
%     Similarly, we also want $q + r > u$ to ensure that the strong learner can't see the spike either. 
%     This verifies \cref{item:spike}. \david{find ref for info theoretic threshold}

%     On the other hand, to ensure that the strong learner fails badly at classification using only the $n$ labeled datapoints, we need 
%     \begin{align}
%         q + r >  \frac{p+1}{2}. \label{eq:strong-fail}
%     \end{align}
%     And note that even if the weak learner had access to the true feature pool, then we would automatically have 
%     \[
%         q_{\weak} + r_{\weak} > \frac{p_{\weak} + 1}{2}. 
%     \]

%     On the other hand, by assumption of the feature model for the weak feature pool, the labels from $f_{\weak}$ are just the true labels with noise level $\frac{1}{2}(1 - \rho)$. 
%     Assuming that $\rho \ge \Omega(1)$, then this implies that the region for generalization for the strong learner trained on the $m$ weakly labeled datapoints is
%     \[
%         q_m + r_m < \frac{1}{2} \cdot (p_m + 1) \iff \frac{q}{u} + \frac{r}{u} < \frac{1}{2} \cdot \qty(\frac{p}{u} + 1) \iff q + r < \frac{p + u}{2}.
%     \]
%     Notice how this does not contradict \eqref{eq:strong-fail} since $u > 1$!
% \end{proof}

% \parhead{Vanishing label noise.} Now let's consider what happens to the strong learner when we allow the labels to be $\rho$-correlated with the truth, where $\rho = o(1)$. 
% Let $\mu_n = n^{1-(q+r)}$ and $\mu_m = m^{1 - (q_m + r_m)} = n^{u - (q+r)}$. 
% By \cite[Lemma 32]{MNS+21}, we have 
%     \[
%         \su \asymp  \rho \mu_m = \rho n^{u - (q+r)}.
%     \]
%     Note that the label noise will always be at least $\Omega(m^{-1/2})$ because of Chernoff, so we may assume that $\nu = n^{-w}$ for some $w \in [0, \frac{u}{2}]$, this gives that 
%     \[
%         \su \asymp n^{u-(q+r) - w} = \mu_m n^{-w}.
%     \]
    
%     % On the other hand, by \cite[Lemma 34, 36]{MNS+21}, we have 
%     % \[
%     %     n^{\frac{1-p}{2}} \lesssim \cn \lesssim  n^{\frac{\min\qty{1-p, r-1}}{2}} \sqrt{\log n}.
%     % \]
%     % This is not tight, and also seems to not depend on the label noise. 
%     % However, the upper bound actually does not depend on the label noise, because the survival will be $o(1)$ as soon as $q+r > 1$, regardless of label noise. 

%     On the other hand, the correct bound from the multiclass paper yields
%     \[
%         \cn \asymp  \mu_m m^{\frac{r_m-1}{2}} + m^{\frac{1-p_m}{2}} = \mu_m n^{\frac{r-u}{2} - w} + n^{\frac{u-p}{2}}.
%     \]
    
%     The corresponding region for generalization, determined by when $\su/\cn = \omega(1)$, then becomes 
%     \[
%             \min\qty{(u-r) - 2w, p+u-2(q+r) - 2w} > 0.
%     \]
%     This makes sense, becuase as the label noise increases it becomes harder for the model to generalize.

%     To summarize, we have proved the following:
%     \begin{proposition}\label{prop:binary-vanishing-label-noise}
%         Suppose that the strong learner is drawn from the $(p, q, r, 0)$-bilevel ensemble scaled to $n$ and that the weak learner is drawn from $(p_{\weak}, q_{\weak}, r_{\weak}, 0)$-bilevel ensemble scaled to $n$. 
%         Assume that the weak learner outputs labels with noise level $\frac{1}{2}(1 - n^{-w})$ for some $w \ge 0$. 
%         Then, the desiderata are satisfied if the following conditions hold:
%         \begin{align*}
%             \max\qty{\frac{p+1}{2} - w, u} &< q + r < \frac{p + u}{2} - w \\
%             w &< \frac{u-r}{2}. \tag*{}
%         \end{align*}
%     \end{proposition}
%     \begin{remark}
%         Observe that twice the label noise level $2w$ essentially plays the same role as the number of classes in the multiclass setting.
%     \end{remark}
% \section{Multiclass classification}
% Now we move onto multiclass classification.
% Define the factor $\mu \triangleq n^{q+r-1}$, so that the asymptotics of $\mu$ mirror whether we can see the spike in the empirical covariance or not. 

% Let us recall the scalings for multiclass classification with true labels. 

% \parhead{Multiclass classification with clean labels.}
% Let us recall the bounds for survival and contamination in the multiclass setting with clean labels. 
% \begin{proposition}[{\cite[Propositions A.1, A.2]{WS24}}]
%     If $q+r>1$ and $k = n^t$ classes for $t \in [0, 1)$, then 
%     \begin{align*}
%         \su &\asymp \mu_n n^{-t} \sqrt{\log k} \\
%         \cn &\lesssim \mu_n n^{\frac{r-t-1}{2}} \log n + n^{\frac{1-t-p}{2}}\sqrt{\log n}.
%     \end{align*}
%     and if we further have either (1) $t > 0$ or (2) $t = 0$ and $q+ r > 1$, then we have a matching lower bound (up to log factors):
%     \begin{align*}
%         \cn \gtrsim \mu_n n^{\frac{r-t-1}{2}} + n^{\frac{1-t-p}{2}}.
%     \end{align*}

% \end{proposition}

%     For clarity, let us simplify the above expressions to pull out the only parts that change when we scale with respect to $m$ instead of $n$:
%     \begin{align*}
%         \su_n &\asymp \mu_n \frac{\sqrt{\log k}}{k} \\
%         \cn_n &\asymp \mu_n \sqrt{\frac{s}{kn}}\log n + \sqrt{\frac{n}{kd}}\sqrt{\log n}. 
%     \end{align*}
%     It follows that (ignoring log factors)
%     \begin{align*}
%         \frac{\su_n}{\cn_n} &\asymp \sqrt{\frac{n}{sk}} + \frac{ad}{s} \sqrt{\frac{nk}{d}} \\
%         &= \sqrt{n}\qty(\frac{1}{\sqrt{sk}} + \lambda_F \sqrt{\frac{k}{d}})
%     \end{align*}

%     Hence, relative to $m = n^u$, we have
%     \begin{align*}
%         \frac{\su_m}{\cn_m} &\asymp n^{u/2} \qty(\frac{1}{\sqrt{sk}} + \lambda_F \sqrt{k}) \\
%         &= n^{u/2} \cdot (n^{-\frac{r+t}{2}} + n^{\frac{p+t}{2}-q-r})
%     \end{align*}

%     % To see how this compares to the binary case, plug in $t=0$ when $q+r>1$ to obtain 
%     % \begin{align*}
%     %     \su &\asymp n^{1-(q+r)} \\
%     %     \cn &\asymp n^{1-(q+r)} n^{\frac{r-1}{2}} + n^{\frac{1-p}{2}}
%     % \end{align*}
    
%     Thus the condition for successful classification with $n^{u}$ \emph{correctly labeled} datapoints is 
%     \begin{align}
%         \Pr[\gE_{\err}[u]] & = \begin{cases} o(1) ,& \ \mathrm{if} \  t < \min\qty{u-r, p+u-2(q+r)} \\
%          1-O\qty(\frac{1}{k^{1-o_k(1)}}),& \ \mathrm{if} \ t > \min\qty{u-r, p+u-2(q+r)}
%          \end{cases}.
%          \label{eq:conjectured_regimes}
%    \end{align}

%    \parhead{Weak to strong generalization for multiclass classification.}
%    We shall assume that the strong learner is in a regime where the error probability is $1 - \Theta(\frac{1}{k})$ using the $n$ correctly labeled datapoints, which is possible whenever 
%    \begin{align*}
%         t > p + 1 - 2(q+r).
%    \end{align*}

%    \begin{assumption}[Weak to strong setup for multiclass]\label{assump:weak-strong-indep}
%     Now suppose that each of the weak features $z_i$ is a $\rho$-correlated version of $x_i$ for $i \in [k]$, where $\rho = n^{-w}$. 
%    The way to model this is to assume that, for $i \in [k]$, we have 
%    \[
%         z_i = \eta(\rho) x_i + g_i,
%    \]
%    where each $g_i$ is an iid standard normal independent of all other random variables. 
%    We also assume that for $j > k$, each $x_j$ and $z_j$ are iid standard normals. 
%    In other words, the only correlations that are exist are those between the weak and strong (true) label defining features.
%    \end{assumption}
%    \begin{theorem}
%     Assume that \Cref{assump:weak-strong-indep} holds. 
%     Using the weak labels with correlation $\rho = n^{-w}$, if 
%     \begin{enumerate}[label=\normalfont{(\arabic*)}]
%         \item $q+r > u$; i.e. the spike can't be seen in the unlabeled data
%         \item $w < \frac{u}{2} - t$; i.e. the label noise is not too high,
%     \end{enumerate}
%     then the survival and contamination relative to $m$ is 
%    \begin{align*}
%         \su_m &\asymp \rho \mu_m \frac{1}{k}\\
%         \cn_m &\asymp \mu_m \sqrt{\frac{s}{km}} + \sqrt{\frac{m}{kd}} \\
%         \frac{\su_m}{\cn_m} &\asymp \rho \sqrt{m} \qty(\frac{1}{\sqrt{sk}} + \lambda_F \sqrt{\frac{k}{d}}) \\
%         &= n^{u/2 - w} \cdot (n^{-\frac{r+t}{2}} + n^{\frac{p+t}{2}-q-r })
%     \end{align*}

%     Consequently, the probability of error for the weakly supervised strong learner satisfies
%     \begin{align}
%         \Pr[\gE_{\err}] & = \begin{cases} o(1) ,& \ \mathrm{if} \  t < \min\qty{u-r, p+u-2(q+r)} - 2w\\
%         1-\Theta(\frac{1}{k}),& \ \mathrm{otherwise}.
%         \end{cases}.
%         \label{eq:conjectured_regimes}
%     \end{align}
%    \end{theorem}

   
